Parallel Ordered Sets Using Join

The ordered set is one of the most important data type in both theoretical algorithm design and analysis and practical programming. In this paper we study the set operations on two ordered sets, including Union, Intersect and Difference, based on four types of balanced Binary Search Trees (BST) including AVL trees, red-black trees, weight balanced trees and treaps. We introduced only one subroutine Join that needs to be implemented differently for each balanced BST, and on top of which we can implement generic, simple and efficient parallel functions for ordered sets. We first prove the work-efficiency of these Join-based set functions using a generic proof working for all the four types of balanced BSTs. We also implemented and tested our algorithm on all the four balancing schemes. Interestingly the implementations on all four data structures and three set functions perform similarly in time and speedup (more than 45x on 64 cores). We also compare the performance of our implementation to other existing libraries and algorithms.

==> exp2.tex <==
\section{Experiments}
\label{sec:exp}
To evaluate the performance of our algorithms we performed several
experiments across the four balancing schemes using different set functions,
while varying the core count and tree sizes.
We also compare the performance of our implementation to other existing libraries and algorithms.
%For the sequential setting we compare ourself to the STL's \texttt{std::set} and \texttt{std::vector},
%while for parallel experiments we compare our code to the MCSTL (Multi Core Standard Template) library \cite{FS07} and
%parallel weight-balanced B-trees (WBB-tree) \cite{WBTree}.

\hide{
We compare the performance of our library on a single core to the C++
Standard Template Library (STL) implementation of ordered maps, which is
based on red-black trees, and their generic implementation of
\union{}.
}
\paragraph{Experiment setups and baseline algorithms}
For the experiments we use a 64-core machine with 4 x AMD Opteron(tm)
Processor 6278 (16 cores, 2.4GHz, 1600MHz bus and 16MB L3 cache). Our code was
compiled using the \texttt{g++} 4.8 compiler with the Cilk Plus
extensions for nested parallelism. The only compilation flag we used was the \texttt{-O2} optimization flag. In all our experiments we use keys
of the double data type. The size of each node is about 40 bytes,
including the two child pointers, the key, the balance
information, the size of the subtree, and a reference count. We
generate multiple sets varying in size from $10^4$ to $10^8$. Depending on the experiment the keys are drawn either from an uniform or a Gaussian distribution.
We use $\mu$ and $\sigma$ to denote the mean and the standard deviation in Gaussian distribution.
Throughout this section $n$ and $m$ represent the two input sizes for functions with two input sets ($n\le m$).


We test our algorithm by comparing it to other available implementations. This includes the sequential version of
the set functions defined in the C++ Standard Template Library (STL)~\cite{musser2009stl} and STL's \texttt{std::set} (implemented by RB tree).
The STL supports the set operations
\texttt{set\_union},
\texttt{set\_intersection}, and
\texttt{set\_difference} on any container class. Using an \texttt{std::vector} these algorithms achieve a runtime of $O(m + n)$.
Since the STL does not offer any parallel version of these functions we could only use it for sequential experiments.
To see how well our algorithm performs in a parallel setting, we compare it to parallel WBB-trees \cite{WBTree} and the MCSTL library \cite{FS07}.
WBB-trees, as well as the MCSTL, offer support for bulk insertions and deletions. They process the bulk updates slighlty different.
The MCSTL first splits the main tree among $p$ processors, based on the bulk sequence, and then inserts the chunks dynamicaly into each subtree.
The WBB-tree recursively inserts the bulk in parallel into the main tree. In order to deal with heavily skewed sequences they
use partial tree reconstruction for fixing imbalances, which takes constant amortized time. The WBB-tree has a more cache aware
layout, leading to a better cache utilization compared to both the MCSTL and our implementation. To make a comparison with these implementations
we use their bulk insertions, which can also be viewed as an union of two sets. However notice that WBB-tree takes the bulk in the form of a sorted 
sequence, which gives them advantage on less accessing time and better cache performance.
\hide{
We perform our experiments with different data distributions, such as the uniform distribution and Gaussian distribution. In the following
we use $\mu$ and $\sigma$ to denote the mean and the standard deviation in the Gaussian distribution.}

\iffalse

\newcommand{\figscale}{0.5}
\begin{figure*}[t!]
\begin{minipage}{.24\textwidth}
  \centering \includegraphics[scale=\figscale]{figures/graphs/tree_comp} \\ (a)
\end{minipage}
\begin{minipage}{.24\textwidth}
\centering \includegraphics[scale=\figscale]{figures/graphs/union_speedup} \\ (b)
\end{minipage}
\begin{minipage}{.24\textwidth}
\centering \includegraphics[scale=\figscale]{figures/graphs/union_speedup2} \\ (c)
\end{minipage}
\begin{minipage}{.24\textwidth}
  \centering \includegraphics[scale=\figscale]{figures/graphs/other} \\ (d)
\end{minipage}

\vspace{.1in}
\begin{minipage}{.24\textwidth}
  \centering \includegraphics[scale=\figscale]{figures/graphs/build} \\ (e)
\end{minipage}
\begin{minipage}{.24\textwidth}
\centering\includegraphics[scale=\figscale]{figures/graphs/union_vs_deunion}\\(f)
\end{minipage}
\begin{minipage}{.24\textwidth}
\centering\includegraphics[scale=\figscale]{figures/graphs/insertion}\\(g)
\end{minipage}
\begin{minipage}{.24\textwidth}
\centering   \includegraphics[scale=\figscale]{figures/graphs/union_sequential}\\(h)
\end{minipage}
%\nocaptionrule
\caption{
(a) Times for \union{} as a function of size ($n = m$) for different
BBSTs;
(b, c) speed up of \union{} for different BBSTs on both of our machines;
(d) times for various operations on AVL trees as a function of size ($m  = 10^8$);
(e) times for different versions of \build{} as a function of size. \union{}-\build{} I is taking a presorted sequence, while
\union{}-\build{} II is taking a permuted one;
(f) Persistent vs. destructive \union{};
and
(g) insertion comparison with the STL;
(h) comparing STLs \texttt{set\_union} with our \union{}
implementation.
}
\label{fig:times}
\end{figure*}

\newcommand{\figscale}{0.65}
\begin{figure*}[t!]
\begin{minipage}{.32\textwidth}
  \centering \includegraphics[scale=\figscale]{figures/new-graphs/compare} \\ (a)
\end{minipage}
\begin{minipage}{.32\textwidth}
\centering \includegraphics[scale=\figscale]{figures/new-graphs/speedup} \\ (b)
\end{minipage}
\begin{minipage}{.32\textwidth}
\centering \includegraphics[scale=\figscale]{figures/new-graphs/operations} \\ (c)
\end{minipage}

\vspace{.1in}

\begin{minipage}{.32\textwidth}
  \centering \includegraphics[scale=\figscale]{figures/new-graphs/union_sequential} \\ (d)
\end{minipage}
\begin{minipage}{.32\textwidth}
\centering\includegraphics[scale=\figscale]{figures/new-graphs/uniform_double}\\(e)
\end{minipage}
\begin{minipage}{.32\textwidth}
  \centering \includegraphics[scale=\figscale]{figures/new-graphs/uniform_string} \\ (f)
\end{minipage}

\vspace{.1in}
\begin{minipage}{.32\textwidth}
\centering\includegraphics[scale=\figscale]{figures/new-graphs/normal_double}\\(g)
\end{minipage}
\begin{minipage}{.32\textwidth}
\centering\includegraphics[scale=\figscale]{figures/new-graphs/deviation}\\(h)
\end{minipage}
\begin{minipage}{.32\textwidth}
\centering\includegraphics[scale=\figscale]{figures/new-graphs/uniform_double_core}\\(i)
\end{minipage}
\caption{
(a) Times for \union{} as a function of size ($m = 10^8$) for different
BBSTs;
(b) speed up of \union{} for different BBSTs;
(c) times for various operations on AVL trees as a function of size ($m  = 10^8$);
(d) comparing STLs \texttt{set\_union} with our \union{};
(e, f, g, h, i) comparing our \union{} to other parallel search trees; (e, i) input keys are uniformly distributed doubles in the range of [0, 1];
(f) input keys are randomly generated strings varying in length between 3 and 20; (g, h) inputs keys follow a normal distribution of doubles -
the mean of the main tree is always $\mu_1=0$, while the mean of the bulk is $\mu_2=1$. Figure (h) uses a standard deviation of $\sigma=0.25$, while
figure (h) shows the performance across different standard deviations.
}
\label{fig:times}
\end{figure*}
\fi

\begin{center}
\begin{figure*}[t!]
\begin{minipage}{.24\textwidth}
  \centering \includegraphics[width=1\columnwidth]{figures/new-graphs/compare} \\ (a)
\end{minipage}
\begin{minipage}{.24\textwidth}
\centering \includegraphics[width=1\columnwidth]{figures/new-graphs/speedup} \\ (b)
\end{minipage}
\begin{minipage}{.24\textwidth}
\centering \includegraphics[width=1\columnwidth]{figures/new-graphs/operations} \\ (c)
\end{minipage}
%\vspace{.1in}
\begin{minipage}{.24\textwidth}
  \centering \includegraphics[width=1\columnwidth]{figures/new-graphs/union_sequential} \\ (d)
\end{minipage}

\vspace{.1in}

\begin{minipage}{.24\textwidth}
\centering\includegraphics[width=1\columnwidth]{figures/new-graphs/uniform_double}\\(e)
\end{minipage}
%\begin{minipage}{.32\textwidth}
%  \centering \includegraphics[scale=\figscale]{figures/new-graphs/uniform_string} \\ (f)
%\end{minipage}
%\vspace{.1in}
\begin{minipage}{.24\textwidth}
\centering\includegraphics[width=1\columnwidth]{figures/new-graphs/normal_double}\\(f)
\end{minipage}
\begin{minipage}{.24\textwidth}
\centering\includegraphics[width=1\columnwidth]{figures/new-graphs/deviation}\\(g)
\end{minipage}
\begin{minipage}{.24\textwidth}
\centering\includegraphics[width=1\columnwidth]{figures/new-graphs/uniform_double_core}\\(h)
\end{minipage}


%\nocaptionrule
\caption{
(a) Times for \union{} as a function of size ($m = 10^8$) for different
BBSTs;
(b) speed up of \union{} for different BBSTs;
(c) times for various operations on AVL trees as a function of size ($m  = 10^8$);
(d) comparing STLs \texttt{set\_union} with our \union{};
(e, f, g, h) comparing our \union{} to other parallel search trees; (e, h) input keys are uniformly distributed doubles in the range of [0, 1];
(f, g) inputs keys follow a normal distribution of doubles -
the mean of the main tree is always $\mu_1=0$, while the mean of the bulk is $\mu_2=1$. Figure (f) uses a standard deviation of $\sigma=0.25$, while
Figure (g) shows the performance across different standard deviations.
}
\label{fig:times}
\end{figure*}
\end{center}

\paragraph{Comparing the balancing schemes and functions}
To compare the four balancing schemes we choose \union{} as the
representative operation. Other operations would lead to similar
results since all operations except \join{} are generic across the
trees. We compare the schemes across different thread counts and different sizes.

Figure~\ref{fig:times} (a) shows the runtime of \union{} for various
tree sizes and all four balancing schemes across 64
cores. The
times are very similar among the balancing schemes---they
differ by no more than 10\%.

Figure~\ref{fig:times} (b) shows the speedup curves for \union{} on varying
core numbers
with two inputs of size $10^8$. All balancing
schemes achieve a speedup of about 45 on 64 cores, and about 30 on 32
cores. The less-than-linear speedup beyond 32 cores is not
due to lack of parallelism, since when we ran the same experiments on
significantly smaller input (and hence less parallelism) we get very
similar curves (not shown). Instead it seems to be due to saturation
of the memory bandwidth.

We use the AVL tree as the representative tree to compare different
functions. Figure~\ref{fig:times} (c) compares the \union{},
\intersect{} and \difference{} functions.  The size of the
larger tree is fixed ($10^8$), while the size of the smaller
tree varies from $10^4$ to $10^8$.
As the plot indicates, the three functions have very similar performance.

The experiments are a good indication of the performance
of different balancing schemes and different functions, while controlling other factors. The
conclusion is that all schemes perform almost equally on all the set functions. It is
not surprising that all balancing schemes achieve similar performance because the dominant cost is in cache misses along the
paths in the tree, and all schemes keep the trees reasonably balanced.
The AVL tree is always slightly faster than the other trees and this
is likely due to the fact they maintain a slightly stricter balance than
the other trees, and hence the paths that need to be traversed are
slightly shorter. For different set functions the performance is also as expected given the similarity of the code.

Given the result that the four balancing schemes do not have a big difference in timing
and speedup, nor do the three set functions, in the following experiments we use the AVL tree along with
\union{} to make comparisons with other implementations.

\par~\par~\par

\paragraph{Comparing to sequential implementations}
The STL supports \texttt{set\_union} on any sorted container class, including sets
based on red-black trees, and sorted vectors (arrays). The STL
\texttt{set\_union} merges the two sorted containers by moving from left to right
on the two inputs, comparing the current values, and writing the lesser
to the end of the output. For two inputs of size $n$ and $m$, $m \ge
n$, it takes $O(m + n)$ time on \texttt{std::vectors}, and $O((n+m) \log (n+m))$
time on \texttt{std::set} (each insertion at the end of the output
red-black tree takes $O(\log(n+m))$ time). In the case of ordered sets we can do better
by inserting elements from the smaller set into the larger, leading a time of $O(n \log (n+m)$.
This is also what we do in our experiments. For vectors we stick with the available \texttt{set\_union} implementation.

  Figure~\ref{fig:times} (d)
gives a comparison of times for \union{}. For equal lengths our implementation is
about a factor of 3 faster than set variant (red-black trees), and about
8 times slower than the vector variant. This is not surprising since we are
asymptotically faster than their red-black tree implementation, and
their array-based implementation just reads and writes the values, one by one,
from flat arrays, and therefore has much less overhead and much
fewer cache misses. For taking the union of smaller and larger inputs,
our \union{} is orders of magnitude faster than either STL version.
This is because their theoretical work bound ($O(m+n)$ and $O(n\log(m+n)$)
is worse than our $O(n \log (m/n))$, which
is optimal in comparison model.
%they both take time proportional to the larger length
%while ours takes $O(n \log (m/n))$  work (time).

\paragraph{Comparing to parallel implementations on various input distributions}
We compare our implementations to other parallel search trees, such as the WBB-trees, as described in \cite{WBTree}, and parallel
RB trees from the MCSTL~\cite{FS07}. We test the performance on different input distributions.

In Figure \ref{fig:times} (e) we show the result of \union{} on uniformly distributed doubles in the range of [0,1] across 64 cores. We set the
input size to $n=m=10^i$, $i$ from $4$ to $8$. The three implementations have similar performance when $m=n=10^4$. As the
input size increases, MCSTL shows much worse performance than the other two because of
the lack of parallelism (Figure \ref{fig:times} (h) is a good indication), and the WBB-tree implementation is slightly better
than ours. Due to the same reason as STL vector outperforms STL set (implemented by RB tree) and our sequential implementation, the WBB-trees takes the bulk as a sorted
sequence, forming better layout which is friendly to many operations and also to the cache. Also their tree layout is more cache efficient and the overall height is lower since they store multiple keys per node.

%Figure \ref{fig:times} (f) shows the result on strings on all 64 cores with set sizes $n=m=10^i$ for $i=4$ through $8$. The strings are of length from 3 through 20, each character
%picked randomly from a to z. The trend of the curves in (f) are very similar to (e).

Figure \ref{fig:times} (f) shows the result of a Gaussian distribution with doubles, also on all 64 cores with set sizes of $n=m=10^i$ for $i=4$ through $8$. The distributions of the two sets have
means at $0$ and $1$ respectively, and both having a standard deviation of $0.25$, meaning that the data in the two sets have less overlap comparing to a uniform distribution (as in (e)). In this case our code achieves better performance than the other two implementations. For our algorithms less overlap in the data means more parts of the trees will be untouched, and therefore less nodes will be operated on. This in turn leads to less processing time.

We also do a in-depth study on how the the overlap of the data sets affects the performance of each algorithm. We generate two sets of size $m=n=10^8$, each from a Gaussian distribution.
The distributions of the two sets have means at $0$ and $1$ respectively, and both have an equal standard deviation varying in $\{1,1/2,1/4,1/8,1/16\}$. The different standard deviations are to control
the overlap of the two sets, and ideally less overlap should simplify the problem. Figure \ref{fig:times} (g) shows the result of the three parallel implementations on a Gaussian distribution with different standard deviations. From the figure we can see that MCSTL and WBB-tree are not affected by different standard deviations, while our join-based union takes the advantage of less overlapping and achieves a much better performance when $\sigma$ is small. This is not surprising since when the two sets are less overlapped, e.g., totally disjoint, our \union{} will degenerate to a simple \join{}, which costs only $O(\log m)$ work. This indicates that our algorithm is the only one among the three parallel implementations that can detect and take advantage of less overlapping in data, hence have a much better performance when the two operated sets are less overlapped.

We also compare the parallelism of these implementations. In Figure \ref{fig:times} (h) we show their performance across 64 cores.
The inputs are both of size $10^8$, and generated from an uniform distribution of doubles.
It is easy to see that MCSTL does not achieve good parallelism beyond 16 cores, which explains why the MCSTL always performs the worst on 64 cores in all settings.
As we mentioned earlier, the WBB-tree are slightly faster than our code, but when it comes to all 64 cores, both algorithms have similar performance. This indicates that our algorithm achieves better parallelism.

To conclude, in terms of parallel performance, our code and WBB-trees are always much better than the MCSTL because of MCSTL's lack of parallelism. WBB-trees achieve a slightly better performance than ours on uniformly distributed data, but it does not improve when the two sets are less overlapped. Thus our code is much better than the other two implementations on less overlapped data, while still achieving a similar performance with the other algorithms when the two sets are more intermixed with each other.



==> imple.tex <==
\section{Library Implementation}
\label{sec:imple}

We have implemented the library using the \join-based approach described in
previous sections for all four balancing schemes (AVL trees, RB trees,
WB trees, and treaps).  The only code that depends on the balancing
scheme are the implementations of \join{}.  For AVL trees we also
directly implemented \insertnew{} for the purposes of
comparison.  Our implementation is in C++ using the \texttt{Cilk-Plus}
extension to support nested parallelism (fork-join using spawn and
sync, and parallel loops).  For our reference counting garbage
collector we also make significant use of compare-and-swap for
lock-free synchronization among the threads.

\paragraph{Implementing persistence.}   
One way to achieve persistence is to copy the entire input before the
function is applied.  This, however, can be much more costly than the
function itself (e.g. for \insertnew{}, \join{}, \split{}).  Instead
we copy the path from the root down to the modification being made.
Figure~\ref{fig:insert} shows an example of such path copying.  All
the nodes along the path that are copied share any pointers to nodes
off the path (in the example both copies of node $5$ share a pointer
to node 8).  In general this means that large parts of trees end up
being shared among different maps.  This is the same approach as used
by default in purely-functional languages.

If all nodes along the path have constant memory size (which is true
in binary trees), path copying only has a constant factor overhead
relative to mutating updates.  This constant, however, has
some practical significance
(we study this cost in our experiments).  Our \texttt{final} function
can be used to avoid this cost.  It allows for in-place updates when
safe.  In particular if the user indicates with \texttt{final} that
this is the final use of a tree, and for any node in the tree that is
not shared with any other trees, that node can be updated in place
rather than requiring a copy.  If the next node(s) in the path is
also updated in place, then no update is needed at all, avoiding some
writes, allocation, and later garbage collection.  The use of
destructive updates on the final copy is a well studied optimization in the
functional programming community~\cite{Hudak86,Wadler90,Odersky91}.

To determine if nodes are shared we use a reference counting collector, which is
described in more detail below.  For now assume that a reference count
of one indicates that there is only one pointer to the structure, and
therefore it is safe to update in place (the only pointer is the one
currently being used).  When entering a function on a map that is not
finalized, the reference count to the root is incremented indicating
that in addition to all existing pointers to the root, the function
itself now has a pointer.   However, when the map is finalized, then
the reference count is left unchanged, indicating that the pointer to the
map is now being handed to the function, and the pointer in the
finalized map is set to empty.    If the count is one, then updates
can be made in place (if not finalized, the reference count will never
be one).     Our map functions include code for updating reference
counts.

\begin{figure}
\centering
  \includegraphics[width=0.95\columnwidth]{figures/Tree_insertion} \\
  \caption{The figure shows the insertion of a node with key 4 into a tree which is shared among two sets. Since
	the root has a reference count of 2 the copying of nodes is propagated along the insertion path. On the last figure
	we fix the reference counts of the nodes which have been copied and adjust the pointers accordingly.}
  \label{fig:insert}
\end{figure}



\paragraph{Reference Counting Collection.}
We use a reference counting garbage collector for memory management of
the tree nodes.  Every node includes a reference count that indicates
the number of references to it, and a node is collected when its count
goes to zero.  The benefit of using a reference counting collector is
twofold.  Firstly, as discussed above, the reference count can detect
nodes that are not shared with any other tree, and can thus be
immediately reused.  This avoids having to allocate a new node, free
the old node, and copy values from the old to the new.  The second
benefit is that nodes can be collected as soon as their count goes to
zero, so that the memory footprint is always almost equal to the
number of reachable (live) nodes.  Since trees do not have cycles,
even when shared, there is no issue with collecting cycles.

Our collector is parallel, safe for concurrency, and lock-free.  We
use compare-and-swap to atomically update all reference counts.  To be
safe for concurrency, the collector also never decrements a counter before
all needed fields are extracted (sequential reference counting can
decrement first since no other thread can see the decrement).  When a
count is decremented to zero, the current thread returns the node to
the memory pool (described below) and recursively decrements the child
pointers.  The decrements could themsleves reduce the counts to zero,
possibly recursively collecting a large portion of the tree.  The
calls are therefore applied in parallel (using nested fork-join), so
the collector is parallel requiring at most $O(\log n)$ span to
collect a balanced tree of size $n$.

We implemented our own memory pool for the nodes.  The nodes are all
the same size, so no provisions are needed for different sized
objects.  To reduce the contention on a shared pool, we use the
standard approach of having each operating system thread maintain its
own local \emph{small stack} of free nodes as a linked list.
Allocations of new nodes are poped from the local small stack, and
freed nodes are pushed onto the local stack.
%all without synchronization as long as there are nodes remaining or 
%the stack is not full.  
In addition we maintain a global pool of small stacks using
a lock-free \emph{global stack}--each stack element is a small stack
of fixed size $s$ (16K nodes in our current version).  Whenever a
local stack runs out of nodes, the thread goes to the global stack and
pops off another small stack of $s$ nodes to use locally.  Also,
whenever a local stack reaches size $2 \times s$, the thread splits
the stack in half, and returns one of the two parts as a small stack
to the global stack.  It keeps the other half as the local stack.
This guarantees that there are at least $s$ push and pop steps on the
local stack before going back to the global stack.  The global stack
is maintained as a linked list accessed through a head structure, which
consists of a pair of adjacent words, the first pointing to the head
of the stack and the second to a version number.  A two-word (16 byte)
compare-and-swap is used to atomically update the pair, always
incrementing the version number.  This avoids locking or the ABA
problem.  The implementation currently aborts when the 64-bit version
number overflows, which would take over 1000 years on a current 64
core system running full tilt.

The user can specify how many nodes they use with the \texttt{reserve}
function, but if they underestimate and the global stack runs out of memory, the
first thread detecting it will initiate the allocation of more space.
New small stacks are constructed in parallel and placed into the
global stack.  This is the only place where threads can block on
another thread---while waiting for the small stacks to be added.


==> interface.tex <==

\section{Library Interface}
\label{interface}

We have defined an implemented a C++ library for ordered sets and maps
based on the ideas presented in previous sections.  The library
supports persistence, is implemented so that aggregate functions run
in parallel, and is safe for concurrency.  The library uses C++
templates to specialize to specific key and value types, and defines
the following structures:
\begin{itemize}
\item \texttt{tree\_set<K>} -- represents an ordered set
\item \texttt{tree\_map<K, V>} -- represents an ordered map
%\item \texttt{augmented\_map<K, V, Op>} -- represents an ordered map
\end{itemize}
where the type \texttt{<K>} must support a comparison function ($<$)
that propertly defines a total order over its elements.  The library
supports maps and sets of different types simultaneously.

\renewcommand{\arraystretch}{1.2}
\begin{table}
\begin{center}
	\begin{tabular}{l|c}
	\hline
	\textit{\textbf{Function}} & \textbf Work, Span \\
	\hline
	\texttt{singleton}, \texttt{size} & $1$ \\
	\hline
	\texttt{insert}, \texttt{delete}, \texttt{find} & $\log n$ \\
	\hline
	\texttt{union}, \texttt{intersect}, \texttt{difference} & $n \log (\frac{m}{n} + 1)$, $\log^2 m$ \\
	\hline
	\texttt{forall} & $n$, $\log n$ \\
	\hline
	\texttt{filter} & $n$, $\log^2 n$ \\
	\hline
	\texttt{build} & $n \log n$, $\log^3 n$ \\
	\hline
	\texttt{split}, \texttt{range} & $\log n$ \\
	\hline
	\texttt{next}, \texttt{previous}, \texttt{first}, \texttt{last} & $\log n$ \\
	\hline
	\texttt{rank}, \texttt{select} & $\log n$ \\
	\hline
	\end{tabular}
	\end{center}
	%\nocaptionrule    
\caption{The core functions in our map and set library and their
      asymptotic costs (all big-O).  For \union{}, \intersect{} and
      \difference{}, $m$ is the size of the larger input, and $n$ of
      the smaller.}
    \label{tab:interface}
\end{table}

The list of core functions along with their costs is given in Table
\ref{tab:interface}.  All functions return their result.  The
interface for maps and sets is almost the same---the map versions of
some of the functions take values as well as keys, or return a value
instead of a flag (for example \split{} on sets returns a boolean, but
\split{} on maps returns an value option).  Also \texttt{forall} only
exists for maps.  Our sets are implemented simply as maps with an
empty value.  In the rest of the discussion we only consider maps.
The library has its own memory manager.  Maps are allocated by the
various map functions that create them, and freed using using
\texttt{clear}.  The library also supplies functions to initialize the
library (\texttt{init}), to reserve some number of nodes
(\texttt{reserve}), and to free the memory when no longer needed
(\texttt{finish}).
% The initialization needs to be called before any
%of the other library functions are called.
The \texttt{reserve} is a
hint for the memory manager, but the library will allocate nodes on
demand if none or not enough were reserved.
%No functions can be called after the \texttt{finish}.

By default all the functions over maps are persistent, meaning that
they do not modify their arguments.  However, the library also gives a
way to specify that one or more arguments are no longer needed when
the function completes.  In particular the user can wrap
\texttt{final} around any map that is an argument to a function, and
when the function is applied it will free (clear) that map.  For
example, \texttt{mapR = union(mapA,mapB)} will create a new map
without modifying \texttt{mapA} or \texttt{mapB}, but \texttt{mapR =
  union(mapA,final(mapB))} will create a new map, leave \texttt{mapA}
as it was, but free \texttt{mapB}.  As described in the next
section, the implementation is careful to only free the nodes that
are not shared among maps.  We note that
\texttt{union(mapA,final(mapB))} is semantically equivalent to
\texttt{union(mapA,mapB); clear(mapB)}, but, as discussed in the next
section, the prior can be more efficient.

\begin{comment}
 However, and obviously, it is
unsafe to call \texttt{clear} or \texttt{final} on a map that is still
being operated on concurrently by any other function.  All results are
fully deterministic independent of interleaving of concurrent tasks
since the functions create new values instead of mutating old ones
(unless final, in which case other copies should no longer be
accessed).
\end{comment}

\begin{comment}
The difference between a tree map and an augmented map is that the latter accepts a binary operator as its thrid argument.
Each node of an augmented map stores the application of the binary operator on the values of the tree rooted at itself.
For this reason augmented maps support an \texttt{accumulate} function. It accepts a key $k'$, and returns the application
of the binary operator on all nodes with a key $k \leq k'$. Table \ref{tab:interface} lists the core functions which are supported by all of our containers.

Most of the functions mentioned in Table \ref{tab:interface} are self-explanatory, and we won't go in much detail into them.
In Table \ref{tab:interface} we didn't list any of the methods which are responsible for allocating and freeing nodes.
The memory allocator is not bound to individual object instances, as it is usually implemented. The reason for this
is that due to persistence two or more objects can share a subset of nodes with each other. The memory allocator we provide
operates on the level of class instances and is accessed through three methods: \texttt{init} is used to initialize the memory allocator of a particular map or set class,
\texttt{reserve} accepts a number $n$ and allocates memory for $n$ nodes, and \texttt{finish} destroys the memory allocator and frees all the memory occupied by it. \\

The method responsible for freeing nodes of individual objects is \texttt{clear}, which effectively empties the content of the container.
\texttt{clear} invokes the garbage collection and recollects all nodes which don't belong to a tree anymore.
\end{comment}

All functions listed in Table~\ref{tab:interface} are safe to call
concurrently even on the same maps.
Another feature of our library is that the map versions of
\texttt{union} and \texttt{intersect} accept a third argument, which
is itself a function.  If any keys appear in both trees, the function
is applied to the corresponding pair of values to generate a new value
to associate with that key.  For example, this can be used to keep a
count for each key, and have union and intersection sum the counts.
By default the function returns its first argument, so that when two
keys are the same in a union or intersection, the first value (from the
argument on the left) is kept.


==> intro.tex <==
\section{Introduction}
\label{intro}
One of the most important aggregate data types used in modern
programming is the set data type, which requires support for
not only lookup, insertion and deletion, but also typical set
operations such as union, intersection and difference. Sets
can either be ordered, with the keys having a total ordering, or
unordered. Ordered sets have the advantage that they additionally
support functions such as reporting the keys within a range or finding
the next key larger than a value. They also have the nice property
that their iteration order is well defined. The lower bound of work
of some basic ordered set operations (such as union, intersect and difference)
under the comparison model
is known to be $\log
{m+n \choose n}=\Theta\left(n\log
  \left(\frac{m}{n}+1\right)\right)$\footnote{Among all $m+n$ elements, there are $m+n \choose n$ possible placements for the $n$ elements from the first set, and hence $\log {m+n \choose n}$  comparisons are necessary to distinguish them.}\footnote{In this paper we use $\log n$ to denote $\log_2 n$.}, where $n$ and $m$ are the sizes of
two sets, $n\le m$. This bound has been met by some sequential algorithms~\cite{hwang1972simple,brown1979fast}.
It has also been achieved by some parallel algorithms \cite{BR98}.

Implementing ordered sets efficiently requires some form of
balanced tree data structure, such as red-black
trees~\cite{redblack}, AVL trees~\cite{avl},
weight-balanced trees~\cite{weightbalanced}, treaps~\cite{SA96},
%2-3 trees, skapegoat trees,
B-trees~\cite{bayer1971binary}, splay trees~\cite{sleator1985self}, or skip-lists~\cite{pugh1990skip}.  Most of these structures support
lookup, insert and delete in logarithmic time.
Conventional operations on balanced BSTs are based on insertion and deletion in sequential order, and it is considerable difficult to process a number of such operations in parallel.
Meanwhile, \insertnew{} and \delete{} each has only one operand, while set functions operate on many elements together.
Considering both the requirement of parallelism and the number of operands,
``batch'' operations such as \join{} and \split{} are more applicable comparing to \insertnew{} and \delete{}.

Tarjan first studied the \join{} and \split{} functions in~\cite{Tarjan83}.
The \join$(L,k,R)$ function takes a key $k$ and two
BSTs $L$ and $R$ such that $k$ is greater than all keys in $L$
and less than all keys in $R$.  It returns the BST containing
$L \cup \{k\} \cup R$. The \split$(T,k)$ function is inverse to \join{}.
It takes a BST $T$ and a key $k$ and returns two BST trees $L$ and $R$ where $L$ contains all keys
in $T$ which are less than $k$ and $R$ contains those larger than $k$. It also returns a bit $b$ indicating
whether $k$ is found in $T$. It is worth noting that \split{} can be built on the top of \join{}.
Tarjan showed how to efficiently implement the
functions on red-black and splay trees but did not give any applications for
the two functions. Adams \cite{adams1992implementing,adams1993functional}
applied \join{} and \split{} on weight balanced trees to some bulk functions
and showed an elegant way to implement \union{}, \intersect{} and \difference{} as
in Figure \ref{fig:unioncode}. The method was then implemented in some languages and libraries
such as MIT/GNU Scheme in Haskell \cite{marlow2010haskell}. Adams claims in his paper that the complexity of these algorithms
has upper bound of $O(m+n)$, which, however, is more than the theoretical lower bound $O\left(n\log (\frac{m}{n}+1)\right)$.
Adams' paper was reported buggy \cite{hirai2011balancing,straka2012adams} in parameter choosing and also in that
the \join{} (which is called \texttt{concat3} in his paper) does not rebalance the tree, but the framework
of set functions implementation is still used and studied today.
Adams did not consider parallelism in the algorithm, but
the divide-and-conquer scheme is inherently parallel.

Blelloch and Miller~\cite{BR98} used \join{} and \split{} on treaps
to generate parallel implementations of \union{}, \intersect{} and
\difference{}, in a similar way as Adams,
and first proved the work-efficiency of these algorithms
by probabilistic analysis on treaps.
They only proved the bound for treaps, and they required the exposed tree,
which is $T_2$ in Figure \ref{fig:unioncode}, to be the tree with the root of higher priority,
which makes the \join{} work trivially $O(1)$. In our version, we do not
specify the exposed tree and prove the bound is still the same, not only for treap, but also for the other
tree structures. Each of the previous work is based on one particular tree structure.
This is because the tree structures may have different balance criteria, leading to different implementations.

In this paper we study the set functions and some other tree functions based on \join{} on four different balanced tree structures including AVL trees, red-black trees, weight-balanced trees and treaps, and to show their theoretical efficiency, i.e., the work of these
functions matches the informational theoretical lower bound under the comparison model. %Specially, the set functions \union{}, \intersect{} and \difference{}
%in Figure \ref{fig:unioncode}
%on two BSTs of size $m$ and $n$ ($m\ge n)$ takes optimal work of $O(n\log(\frac{m}{n}+1))$.
Though the set functions (\union{}, \intersect{} and \difference{}) as shown in Figure \ref{fig:unioncode}
have been studied over years, to the best of our knowledge,
no one has explicitly proved its work-efficiency
for various balancing schemes and set functions.
Actually, in previous works, only some incomplete analysis is provided, such as a loose bound
($O(m+n)$ in \cite{adams1992implementing,adams1993functional}),
a proof with stronger assumptions
(assumed perfect-balance in \cite{lecturenote}),
or proofs on a particular balance scheme (treaps in \cite{BR98}, weight-balanced
trees in \cite{adams1992implementing,adams1993functional}).
In this paper, we provide a new and simple proof working
for all the four balance schemes (AVL trees, red-black trees, weight-balanced
trees and treaps) and all three
functions (\union{}, \intersect{} and \difference{}).
%We note that the bound $O(n\log(\frac{m}{n}+1))$ is sublinear in the sum of the two input sizes.
Furthermore all bulk functions in this paper are highly parallel, all with
polylogarithmic span, and very space-efficient, which can be done totally in-place with $O(1)$ extra space.

The optimality of the set functions based on \join{} allows us to build a efficient and generic parallel framework on set implementations
using a variety of balanced BST data structures.
The framework is based on using the \emph{single} function \join{} that needs to be implemented for each
data structure and then building all other functions on top of it.
As introduced above, the \join{} function returns an ordered set as a balanced BST, which means some rebalancing mechanism is required.
Therefore different tree structures will necessarily have different \join{} subroutines. An
important observation is that the balance criteria of a tree is \emph{fully}
captured by how two trees are joined, and all other operations could be identical
over different tree structures. We describe efficient \join{} algorithms for each of
the four tree structures. Then by utilizing \join{}, we design other tree functions such as \split{}, \build{}, \insertnew{}
and \delete{}, as well as set functions \union{}, \intersect{} and \difference{}
with generic code across all different balancing schemes. The work of these
functions based on \join{} is optimal, i.e.,
$O(\log n)$ for \split{}, \insertnew{} and
\delete{} on a tree of size $n$, $O(n\log n)$ for \build{} on an array of size $n$
and $O(n\log(\frac{m}{n}+1))$ for \union{}, \intersect{} and \difference{}
on two trees of size $m$ and $n$ ($n\le m$).

To conclude, the contributions of the paper can be summarized as follows.
1) We propose \join{} functions on AVL trees, red-black trees, weight-balanced
trees and treaps, based on which we can build generic framework across all these
tree structures implementing a variety of functions including \insertnew{}, \delete,
\split, \union, \intersect, \difference{} and so on; 2) we provide a generic
and simple proof for the work-efficiency on three set functions \union{}, \intersect{} and
\difference{} across all four tree structures; and 3) we study the
performance of our approach by comparing different tree
structures, various set operations, and by comparing our implementation to other parallel search trees.

  % and accessors for the key
  % (and value for maps), left subtree and right subtree of a node.


\newcommand{\tr}[2]{T_{#1}^{#2}}

\begin{figure}[!h!t]
\begin{lstlisting}[numbers=none,frame=lines]
union($T_1$,$T_2$) =
  if $T_1$ = Leaf then $T_2$
  else if $T_2$ = Leaf then $T_1$
  else ($L_2$,$k_2$,$R_2$) = expose($T_2$);
    ($L_1$,$b$,$R_1$) = split($T_1$,$k_2$);
    ($\Tl$,$\Tr$) = union($L_1$,$L_2$) || union($R_1$,$R_2$);
    join($\Tl$,$k_2$,$\Tr$) @\vspace{.1in}@
intersect($T_1$,$T_2$) =
  if $T_1$ = Leaf then Leaf
  else if $T_2$ = Leaf then Leaf
  else ($L_2$,$k_2$,$R_2$) = expose($T_2$);
    ($L_1$,$b$,$R_1$) = split($T_1$,$k_2$);
    ($\Tl$,$\Tr$) = intersect($L_1$,$L_2$) || intersect($R_1$,$R_2$);
    if $b$ = true then join($\Tl$,$k_2$,$\Tr$)
    else join2($\Tl$,$\Tr$) @\vspace{.1in}@
difference($T_1$,$T_2$) =
  if $T_1$ = Leaf then Leaf
  else if $T_2$ = Leaf then $T_1$
  else ($L_2$,$k_2$,$R_2$) = expose($T_2$);
    ($L_1$,$b$,$R_1$) = split($T_1$,$k_2$);
    ($\Tl$,$\Tr$) = difference($L_1$,$L_2$) || difference($R_1$,$R_2$);
    join2($\Tl$,$\Tr$)
\end{lstlisting}
\caption{Implementing \union{}, \intersect{} and \difference{} with \join.  \split$(T,k)$
  splits the BST $T$ at the key $k$, returning
  the two sides and a flag indicating whether the key was found (not
  used here), which can be implemented with just \join{}
  in $O(\log n)$ time (Section~\ref{sec:operations}). \joinTwo{} is similar to \join{} but without the
  intermediate key.
  \expose{} is to break the tree into the left subtree, the root, and the right subtree. The syntax $e_1~||~e_2$ means that the expressions $e_1$ and $e_2$ can run in parallel and
return a pair of results when both are done.
  }
\label{fig:unioncode}
\end{figure}


\paragraph{Related Work}
Merging two ordered sets has been well studied. Hwang and Lin \cite{hwang1972simple}
describe an algorithm to merge two arrays, which costs optimal work. Their algorithm works
for arrays, and since writing back both array costs $O(m+n)$ work, the algorithm only returns
the cross pointers between two arrays. Brown and Tarjan \cite{brown1979fast} considered input data
to be arranged in a BST, which allows the merged result to be explicitly given by a new BST in time \bound{}.
Their algorithm works on AVL and 2-3 trees. None of these algorithms considered parallelism. Katajainen et al. \cite{katajainen1992space}
studied the space-efficiency on merging two sets in parallel. Their focus is not on reducing time complexity.
Furthermore the above-mentioned works are not
based on join and are much more complicated than our algorithm.

\join{} and \split{} appear
in the LEDA library~\cite{Leda99} for sorted sequences, and the CGAL
library for ordered maps~\cite{Wein05}.  None of this work considered
parallel algorithms based on the functions, nor how to build an
interface out of just \join{}. Frias and Singler~\cite{FS07} use \join{} and \split{}
on red-black trees for an implementation of the MCSTL, a multicore version of the C++ Standard
Template Library (STL).  Their algorithms are lower level based on
partitioning across processors, and are for bulk insertion and
deletion.

Several researchers have studied how to implement aggregate functions
on balanced trees in parallel.  Paul, Vishkin, and Wagener studied
bulk insertion and deletion on 2-3 trees in the PRAM
model~\cite{PVW83}.  Park and Park showed similar results for
red-black trees~\cite{PP01}. There are also plenty of research on set operations based on multiway split and join.
Katajainen~\cite{katajainen1994efficient} introduced union algorithm with optimal work and $O(\log m)$ span,
but the algorithm is buggy and the bound dos not hold in that version. Yaroslav Akhremtsev and Peter Sanders \cite{??}
introduced efficient and practical set functions implemented by (a,b)-trees, which is optimal in work. These algorithms are based on particular
trees, are not based on a two-way \join{}.

\hide{
\subsection{Old}

A Binary Search Tree (BST) is a binary tree data structure which keeps its keys in sorted order, i.e., the in-order of the tree should be a sorted list. It provides very convenient interface for searching, inserting and deleting, with time complexity of $O(h(T))$. A BST is an efficient data structure for storing and searching ordered data. A BST with $n$ keys has the lower bound of height of $\log n$, and could degenerate to a linked list in the worst case, where the costs of searching and inserting are both $O(n)$. Thus in practice, BSTs are necessary to be organized in a balanced structure, where the left subtree and the right subtree of a certain node do not differ too much in height. Generally speaking, a Balanced BST (BBST) refers to BSTs with bounded height of $O(\log n)$ (or has a height bounded by $O(\log n)$ w.h.p.\footnote{We use ``with high probability'' (w.h.p.) to mean probability at least $1-n^{-c}$ for any constant $c>0$.} for randomized BSTs). Balanced BSTs are widely used in sorting, file systems, databases and geometry algorithms. Balanced BST is also a efficient way to implement and maintain some structures requiring ordering, such as priority queues and ordered sets. In this paper, we focus on ordered sets implemented by BBSTs.

Conventional operations on balanced BSTs are based on insertion and deletion, which are both essentially sequential, and hard to be parallelized. From a parallel perspective, instead of \texttt{insert} and \texttt{delete}, some ``batch'' operations such as \texttt{join} and \texttt{split} are more applicable. In this paper, we use \texttt{join} as the basic operation, and give efficient algorithm of \texttt{join} on four typical BSTs: AVL, red-black tree, treap and weight balanced tree. With \texttt{join} as subroutine and another sequential tool \texttt{split} deriving from \texttt{join}, and further discuss the implementation of other tree operations, which are not dependent on BST types, such as building a tree from the associate array, splitting a tree by a key, getting the union, intersection or difference of two trees. All these are basic and frequently-used operations for BSTs and are also essential for BST's application on ordered sets. By applying \texttt{join}, all these operations can be highly-paralleled with a work of theoretical lower bound and a polylogarithmic depth. Also, other basic tree operations, such as insertion and deletion, can also be done sequentially within time no more than the conventional implementation, i.e., $O(\log N)$.

In this paper, we design algorithms for basic tree operation based on the \texttt{join} paradigm. This framework helps tree operations easy to be paralleled. For four most commonly used balanced BSTs, i.e., AVL, red-black tree, treap and weight-balanced tree, we theoretically prove the \texttt{build} operation can be done with $O(N\log N)$ work and $O(\log^3 N)$ depth, whereas \texttt{merge} (or \texttt{union}), \texttt{intersect} and \texttt{difference} two trees of size $M$ and $N$ ($N<M$) takes work $O\left(N\log(\frac{M}{N}+1)\right)$ and depth of $O(\log M \log N)$. For general insertion and deletion, the implementation based on \texttt{split} and \texttt{join} still takes time $O(\log N)$. All these algorithms are work-efficient. We also implement our algorithm and build a library on persist set operations, and apply it on some real-world settings. We test it on a 40-core (with two-way hyper-threading) machine and get a speedup at up to 58. Experiments show that our algorithm provides efficient interfaces for parallel.

The organization of this paper is as follows. Section \ref{preli} prepares preliminary of this paper. Section \ref{paradigm} briefly introduces the basic paradigms \texttt{join}. Section \ref{operation} describes the detail the other operations based on them. Section \ref{imple} explains some key issue in implementing the persist set operation library. Then in Section \ref{exp} we show the result of our experiment to show the superiority of our algorithms. In Section \ref{conclusion}, we conclude this paper.
}

